Identification of Subgroups With Similar Benefits in Off-Policy Policy Evaluation

Off-policy policy evaluation methods for sequential decision making can be used to help identify if a proposed decision policy is better than a current baseline policy. However, a new decision policy may be better than a baseline policy for some individuals but not others. This has motivated a push towards personalization and accurate per-state estimates of heterogeneous treatment effects (HTEs). Given the limited data present in many important applications, individual predictions can come at a cost to accuracy and confidence in such predictions. We develop a method to balance the need for personalization with confident predictions by identifying subgroups where it is possible to confidently estimate the expected difference in a new decision policy relative to a baseline. We propose a novel loss function that accounts for uncertainty during the subgroup partitioning phase. In experiments, we show that our method can be used to form accurate predictions of HTEs where other methods struggle.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Refer to section \ref{sec:conc} to last two paragraphs.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Refer to section \ref{sec:conc}, where we discuss over reliance on our results.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Refer to supplementary materials for details.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Refer to supplementary materials for details.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code is provided in the supplementary materials. Instruction on how to access data/ simulator is provided in the referenced publications.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Some in the main text, all details can be found in the supplementary materials.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{Our method is not computationally intensive, and we used a normal personal computer to obtain the results.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{MIMIC dataset and Sepsis simulator, both referenced in the main text.}
  \item Did you mention the license of the assets?
    \answerNA{All are publicly accessible.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{MIMIC dataset does not include any personal identifiers.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> theorem1.tex <==

\begin{theorem}\label{th:loss}
    Let $T(x;L)$ be the group treatment effect defined in equation
    \ref{eq:group_treatment_effect}, $t(x)$ be the individual
    treatment effect and $\hat{T}(x;L)$ an unbiased estimator of
    $T(x;L)$. The following inequality holds for the empirical adjusted MSE defined in equation \ref{eq:empirical_amse}
    over a dataset $\mathcal{D}$,
    \begin{align}\label{eq:theorem}
        \nonumber EMSE&(\hat{T}) \leq \\ &-\frac{1}{N}\sum_{i=1}^N \hat{T}^2(x_i;L) + \frac{2}{N}\sum_{i=1}^N \mathbb{V}\left[\hat{T}(x_i;L) \right]
    \end{align}
    Where $\mathbb{V}[\hat{T}]$ is the variance
    of the estimator $\hat{T}$ and $N$ is the total number of samples.
\end{theorem}
\begin{align*}
    AMSE(\hat{T}) = \underset{x\sim\mathcal{X}}{\mathbb{E}} \left[\left(t(x) - \hat{T}(x; L)\right)^2 - t(x)^2\right]
\end{align*}
\begin{eqnarray}
    AMSE(\hat{T}) &=&  \underset{x\sim\mathcal{X}}{\mathbb{E}} \left[\left(t(x) - \hat{T}(x; L)\right)^2 - t(x)^2\right] \\
    &=&  \underset{x\sim\mathcal{X}}{\mathbb{E}} \left[\left(t(x) - T(x;L) + T(x;L) - \hat{T}(x; L)\right)^2 - t(x)^2\right] 
    \end{eqnarray}
% \begin{proof}
% See slides 149-150 (from Ramtin's slide deck)  
% https://docs.google.com/presentation/d/1YgiozHSvLiNaDhh0PLmVE9BLk-zpmN1SxJfkWZP1dj0/edit#slide=id.gb188c4c914_0_150

% \end{proof}
